Large Wireless Localization Model (LWLM): A Foundation Model for Positioning in 6G Networks

Accurate and robust localization is a critical enabler for emerging 5G and 6G applications, including autonomous driving, extended reality (XR), and smart manufacturing. While data-driven approaches have shown promise, most existing models require large amounts of labeled data and struggle to generalize across deployment scenarios and wireless configurations. To address these limitations, we propose a foundation-model-based solution tailored for wireless localization. We first analyze how different self-supervised learning (SSL) tasks acquire general-purpose and task-specific semantic features based on information bottleneck (IB) theory. Building on this foundation, we design a pretraining methodology for the proposed Large Wireless Localization Model (LWLM). Specifically, we propose an SSL framework that jointly optimizes three complementary objectives: (i) spatial-frequency masked channel modeling (SF-MCM), (ii) domain-transformation invariance (DTI), and (iii) position-invariant contrastive learning (PICL). These objectives jointly capture the underlying semantics of wireless channel from multiple perspectives. We further design lightweight decoders for key downstream tasks, including time-of-arrival (ToA) estimation, angle-of-arrival (AoA) estimation, single base station (BS) localization, and multiple BS localization. Comprehensive experimental results confirm that LWLM consistently surpasses both model-based and supervised learning baselines across all localization tasks. In particular, LWLM achieves 26.0%--87.5% improvement over transformer models without pretraining, and exhibits strong generalization under label-limited fine-tuning and unseen BS configurations, confirming its potential as a foundation model for wireless localization.

==> IEEEabrv.tex <==


% IEEE Journals


% aerospace and military
% @STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
% @STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
% @STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
% @STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
% @STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
% @STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
% @STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
% @STRING{IEEE_J_IV         = "{IEEE} Trans. Intell. Veh."}
% @STRING{IEEE_J_TTE        = "{IEEE} Trans. Transport. Electrific."}
% @STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}
% @STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}



% circuits, signals, systems, audio and controls
% @STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
% @STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
% @STRING{IEEE_J_SYST       = "{IEEE} Syst. J."}
% @STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
% @STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
% @STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
% in 2014 ASL became ASLP
% @STRING{IEEE_J_ASLP       = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
% @STRING{IEEE_J_ASL        = "{IEEE} Audio, Speech, Language Process."}
% @STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
% @STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
% @STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
% @STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
% @STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
% @STRING{IEEE_J_ETCAS      = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
% @STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
% @STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
% @STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
% @STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
% @STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



% communications
% @STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
% @STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
% @STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
% @STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
% @STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}
% @STRING{IEEE_J_WCOML      = "{IEEE} Wireless Commun. Lett."}



% components, packaging and manufacturing
% @STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
% @STRING{IEEE_J_CHMT       = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
% in 2011 CAPT became CPMT
% @STRING{IEEE_J_CPMT       = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
% @STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
% @STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
% @STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
% @STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon. Packag. Technol."}
% @STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag. Technol."}
% @STRING{IEEE_J_CPART      = "{IEEE} Trans. Compon. Parts"}
% @STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manuf."}
% @STRING{IEEE_J_MFT        = "{IEEE} Trans. Manuf. Technol."}
% @STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
% @STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
% @STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided Design"}
% @STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}



% coding, data, information, knowledge
% @STRING{IEEE_J_BD         = "{IEEE} Trans. Big Data"}
% @STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
% @STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
% @STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



% computers, computation, networking and software
% @STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
% @STRING{IEEE_J_ES         = "{IEEE} Embedded Syst. Lett."}
% @STRING{IEEE_J_IOT        = "{IEEE} Internet Things J."}
% @STRING{IEEE_J_XCDC       = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
% @STRING{IEEE_J_MMCT       = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
% @STRING{IEEE_J_SUSC       = "{IEEE} Sustain. Comput."}
% @STRING{IEEE_J_CC         = "{IEEE} Trans. on Cloud Comput."}
% @STRING{IEEE_J_CSS        = "{IEEE} Trans. Comput. Social Syst."}
% @STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
% @STRING{IEEE_J_CNS        = "{IEEE} Trans. Control Netw. Syst."}
% @STRING{IEEE_J_DSC        = "{IEEE} Trans. Depend. Sec. Comput."}
% @STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
% @STRING{IEEE_J_ETC        = "{IEEE} Trans. Emerg. Topics Comput."}
% @STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
% @STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% @STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
% @STRING{IEEE_J_MSCS       = "{IEEE} Trans. Multi-Scale Comput. Syst."}
% @STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
% @STRING{IEEE_J_NSE        = "{IEEE} Trans. Netw. Sci. Eng."}
% @STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
% @STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
% in 2012 NN became NNLS
% @STRING{IEEE_J_NNLS       = "{IEEE} Trans. Neural Netw. Learn. Syst."}
% @STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
% @STRING{IEEE_J_SC         = "{IEEE} Trans. Serv. Comput."}
% @STRING{IEEE_J_SIPN       = "{IEEE} Trans. Signal Inf. Process. Netw."}
% @STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



% computer graphics, imaging, and multimedia
% @STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
% @STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
% @STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
% @STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, artificial intelligence and automation
% @STRING{IEEE_J_JAS        = "{IEEE/CAA} J. Autom. Sinica"}
% @STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
% @STRING{IEEE_J_AFFC       = "{IEEE} Trans. Affect. Comput."}
% @STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
% @STRING{IEEE_J_AMD        = "{IEEE} Trans. Auton. Mental Develop."}
% @STRING{IEEE_J_CCN        = "{IEEE} Trans. on Cogn. Commun. Netw."}
% in 2015 AMD became CDS
% @STRING{IEEE_J_CDS        = "{IEEE} Trans. Cogn. Develop. Syst."}
% @STRING{IEEE_J_CIAIG      = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
% in 2013 SMCB became CYB
% @STRING{IEEE_J_CYB        = "{IEEE} Trans. Cybern."}
% @STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
% @STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
% in 2013 SMCC became HMS
% @STRING{IEEE_J_HMS        = "{IEEE} Trans. Human-Mach. Syst."}
% @STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
% @STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
% in 1989 JRA became RA
% in August 2004, RA split into ASE and RO
% @STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
% @STRING{IEEE_J_RAL        = "{IEEE} Robot. Autom. Lett."}
% @STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
% @STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
% @STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
% @STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
% @STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
% in 2012 SMCA became SMCS
% @STRING{IEEE_J_SMCS       = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
% @STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



% earth, wind, fire and water
% @STRING{IEEE_J_GRSL       = "{IEEE} Geosci. Remote Sens. Lett."}
% @STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
% @STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
% @STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}
% @STRING{IEEE_J_STARS      = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}



% education, engineering, history, IEEE, professional
% @STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
% @STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
% @STRING{IEEE_J_RITA       = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
% @STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
% @STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
% @STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
% @STRING{IEEE_J_LT         = "{IEEE} Trans. Learn. Technol."}
% @STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
% @STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
% @STRING{IEEE_J_MAGL       = "{IEEE} Magn. Lett."}
% @STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
% @STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
% @STRING{IEEE_J_RFIC       = "{IEEE} {RFIC} J."}
% @STRING{IEEE_J_RFID       = "{IEEE} {RFID} J."}
% @STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
% @STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
% @STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
% @STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Techn."}
% @STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
% @STRING{IEEE_J_TTHZ       = "{IEEE} Trans. {THz} Sci. Technol."}
% @STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy, power and conversion
% @STRING{IEEE_J_PHOT       = "{IEEE} J. Photovolt."}
% @STRING{IEEE_J_PEL        = "{IEEE} Power Electron. Lett."}
% @STRING{IEEE_J_PETS       = "{IEEE} Power Energy Technol. Syst. J."}
% @STRING{IEEE_J_ESTPE      = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
% @STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}
% @STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
% @STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}
% @STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
% @STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}
% @STRING{IEEE_J_SG         = "{IEEE} Trans. Smart Grid"}
% @STRING{IEEE_J_STE        = "{IEEE} Trans. Sustain. Energy"}



% industrial, commercial and consumer
% @STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}
% @STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
% @STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% @STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
% @STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
% @STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
% @STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
% @STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
% @STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
% @STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}



% instrumentation and measurement
% @STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% @STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
% @STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielectr. Electr. Insul."}
% @STRING{IEEE_J_EI         = "{IEEE} Trans. Electr. Insul."}



% mechanical
% @STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}
% in 2014 MEMS became MEMSI
% @STRING{IEEE_J_MEMSI      = "J. Microelectromech. Syst."}
% @STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatronics"}



% medical and biological
% @STRING{IEEE_J_BHI        = "{IEEE} J. Biomed. Health Inform."}
% @STRING{IEEE_J_TEHM       = "{IEEE} J. Transl. Eng. Health Med."}
% @STRING{IEEE_J_LS         = "{IEEE} Life Sci. Lett."}
% @STRING{IEEE_J_RBME       = "{IEEE} Rev. Biomed. Eng."}
% @STRING{IEEE_J_BCAS       = "{IEEE} Trans. Biomed. Circuits Syst."}
% @STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
% B-ME later dropped the hyphen and became the BME
% @STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% @STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
% @STRING{IEEE_J_CBB        = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
% @STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
% @STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
% @STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% @STRING{IEEE_J_MBSC       = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
% @STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
% @STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
% @STRING{IEEE_J_RE         = "{IEEE} Trans. Rehabil. Eng."}



% optics, lightwave and photonics
% @STRING{IEEE_J_JLT        = "J. Lightw. Technol."}
% @STRING{IEEE_J_OCN        = "{IEEE} J. Opt. Commun. Netw."}
% @STRING{IEEE_J_PJ         = "{IEEE} Photon. J."}
% @STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
% @STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
% @STRING{IEEE_J_EDS        = "{IEEE} J. Electron Devices Soc."}
% @STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
% @STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum Electron."}
% @STRING{IEEE_J_ENANO      = "{IEEE} Nanotechnol. Express"}
% @STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
% @STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
% @STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
% @STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% @STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}
% @STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% @STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochem. Solid-State Lett."}
% @STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
% @STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Supercond."}
% @STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond. Manuf."}



% sensors
% @STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
% @STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





% IEEE Magazines and Online Publications


% @STRING{IEEE_O_ACC        = "{IEEE} Access"}
% @STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
% @STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
% @STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
% @STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
% @STRING{IEEE_M_CHINAC     = "China Commun."}
% @STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
% @STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
% @STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
% @STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% @STRING{IEEE_O_CSTO       = "{IEEE} Commun. Surveys Tuts."}
% @STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
% CSEM changed to CSE in 1999
% @STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
% @STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
% @STRING{IEEE_M_C          = "Computer"}
% @STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
% @STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
% @STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
% @STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
% in 2012 DTC became DT
% @STRING{IEEE_M_DT         = "{IEEE} Des. Test"}
% @STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
% @STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
% @STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
% @STRING{IEEE_M_ETF        = "{IEEE} Electrific. Mag."}
% @STRING{IEEE_M_EMC        = "{IEEE} Electromagn. Compat."}
% @STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
% @STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
% @STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
% @STRING{IEEE_M_EXP        = "{IEEE} Expert"}
% @STRING{IEEE_M_GRS        = "{IEEE} Geosci. Remote Sens. Mag."}
% @STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
% @STRING{IEEE_M_IE         = "{IEEE} Ind. Electron. Mag."}
% @STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
% @STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
% @STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
% @STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
% @STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
% @STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
% @STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
% @STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
% @STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol. Mag."}
% @STRING{IEEE_M_NET        = "{IEEE} Netw."}
% IEEE's editorial manual lists "Pers. Commun.",
% but "Personal Commun. Mag." seems to be what is used in the journals
% @STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
% @STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
% @STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% @STRING{IEEE_M_PEL        = "{IEEE} Power Electron. Mag."}
% CAP and PER merged to form PE in 2003
% @STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
% @STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
% @STRING{IEEE_M_PULSE      = "{IEEE} Pulse"}
% @STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
% @STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
% @STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
% @STRING{IEEE_M_S          = "{IEEE} Softw."}
% @STRING{IEEE_M_SSC        = "{IEEE} Solid-State Circuits Mag."}
% @STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
% @STRING{IEEE_M_SMC        = "{IEEE} Syst., Man, Cybern. Mag."}
% @STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
% @STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
% @STRING{IEEE_M_WC         = "{IEEE} Wireless Commun."}
% @STRING{IEEE_M_TODAY      = "Today's Engineer"}

% % Journal
% % COMST:IEEE Commun. Surveys Tuts.
% % TSP:  IEEE Trans. Signal Process.
% % TWC:  IEEE Trans. Wireless Commun.
% % TCOM: IEEE Trans. Commun.
% % JSAC: IEEE J. Sel. Areas Commun.
% % JSTSP:IEEE J. Sel. Topics Signal Process.
% % ISJ:  IEEE Syst. J.
% % ITS:  IEEE Trans. Intell. Transp. Syst.
% % MTT:  IEEE Trans. Microw. Theory Techn.
% % TMC:  IEEE Trans. Mobile Comput.
% % TIM:  IEEE Trans. Instrum. Meas.


% % Letter 
% % WCL:  IEEE Wireless Commun. Lett.
% % Magazine
% % SP magazine: IEEE Signal Process. Mag.
% % Com mag.
% % Open Journal
% % OJ-COMS: IEEE Open J. Commun. Soc.
% % OJVT: IEEE Open J. Veh. Technol.

% % Conf.
% % EuCAP:    Proc. Eur. Conf. Antennas Propag. (EuCAP)
% % GLOBECOM: Proc. IEEE Global Commun. Conf. (GLOBECOM)
% % ICASSP:   Proc. IEEE Int. Conf. Acoust., Speech, Signal Process. (ICASSP)
% % ICC:      Proc. IEEE Int. Conf. Commun. (ICC)
% % VTC:      IEEE Veh. Technol. Conf. (VTC)
% % WCNC:     Proc. IEEE Wireless Commun. Netw. Conf. (WCNC)
% % PIMRC:    Proc. Annu. Int. Symp. Pers. Indoor Mobile Radio Commun. (PIMRC)
% % InfoCOM:  Proc. IEEE Conf. Comput. Commun. (INFOCOM)
% % EUCNC:    Eur. Conf. Netw., Commun. (EuCNC)
% --
% EOF


==> acronyms.tex <==
% \newlist{acronyms}{description}{1}
% \setlist[acronyms]{
% labelwidth = 4.5em,
% leftmargin = 5em,
% noitemsep,
% itemindent = 0pt}
% \DeclareAcroListStyle{mystyle}{list}{ list = acronyms }
% \acsetup{ list-style = mystyle }








% \acrodef{ad}[AD]{autonomous drive}
\acrodef{6g}[6G]{the sixth generation}
% \acrodef{adas}[ADAS]{advanced driver assistance system}
\acrodef{aoa}[AOA]{angle-of-arrival}
% \acrodef{aod}[AOD]{angle-of-departure}
% \acrodef{ap}[AP]{access point}
\acrodef{bs}[BS]{base station}
\acrodef{bse}[BSE]{beam squint effect}
% \acrodef{cdf}[CDF]{cumulative distribution function}
\acrodef{crb}[CRB]{Cram\'er-Rao bound}
% \acrodef{cpu}[CPU]{central processing unit}
% \acrodef{coa}[COA]{curvature of arrival}
% \acrodef{dbscan}[DBSCAN]{density-based spatial clustering of applications with noise}
% \acrodef{dof}[DOF]{degrees-of-freedom}
\acrodef{elaa}[ELAA]{extremely large antenna array}
\acrodef{ff}[FF]{far-field}
% \acrodef{gdop}[GDOP]{geometric dilution of precision}
% \acrodef{gnss}[GNSS]{global navigation satellite system}
% \acrodef{gps}[GPS]{global positioning system}
% \acrodef{imu}[IMU]{inertial measurement unit}
% \acrodef{ip}[IP]{incidence point}
% \acrodef{kpi}[KPI]{key performance indicator}
\acrodef{las}[L\&S]{localization and sensing}
\acrodef{los}[LOS]{line-of-sight}
% \acrodef{mae}[MAE]{mean absolute value}
% \acrodef{map}[MAP]{maximum a posteriori}
% \acrodef{mle}[MLE]{maximum likelihood estimator}
% \acrodef{ml}[ML]{machine learning}
% \acrodef{mpc}[MPC]{multipath component}
% \acrodef{music}[MUSIC]{multiple signal classification}
\acrodef{nf}[NF]{near-field}
\acrodef{nlos}[NLOS]{non-line-of-sight}
\acrodef{ofdm}[OFDM]{orthogonal frequency division multiplexing}
% \acrodef{prs}[PRS]{positioning reference signal}
% \acrodef{pss}[PSS]{primary synchronization signal}
% \acrodef{ps}[PS]{phase shifter}
% \acrodef{pwm}[PWM]{planar wave model}
% \acrodef{rf}[RF]{radio frequency}
% \acrodef{rfc}[RFC]{radio frequency chain}
\acrodef{ris}[RIS]{reconfigurable intelligent surface}
% \acrodef{rss}[RSS]{received signal strength}
% \acrodef{rtk}[RTK]{real-time kinematic}
% \acrodef{rtt}[RTT]{round-trip-time}
% \acrodef{slam}[SLAM]{simultaneous localization and mapping}
% \acrodef{sinr}[SINR]{signal-to-interference-plus-noise ratio}
% \acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{sns}[SNS]{spatial non-stationarity}
% \acrodef{ssb}[SSB]{synchronization signal/physical broadcast channel block}
\acrodef{swm}[SWM]{spherical wave model}
% \acrodef{tdoa}[TDOA]{time-difference-of-arrival}
% \acrodef{toa}[TOA]{time-of-arrival}
% \acrodef{ttd}[TTD]{true-time delay}
\acrodef{siso}[SISO]{single-input single-output}
\acrodef{ue}[UE]{user equipment}
% \acrodef{ura}[URA]{uniform rectangular array}
% \acrodef{ula}[ULA]{uniform linear array}
% \acrodef{va}[VA]{virtual anchor}
% \acrodef{xlmimo}[XL-MIMO]{extra large multiple-input-multiple-output}
\acrodef{dmimo}[D-MIMO]{distributed MIMO}
\acrodef{MIMO}[MIMO]{multi-input multi-output}
% \acrodef{rs}[RS]{radio stripe}
% \acrodef{cf}[CF]{cell-free}
% \acrodef{peb}[PEB]{position error bound}


















% Abbreviations for Conferences
% @STRING{ICASSP         = "Proc. IEEE Int. Conf. Acoustics, Speech, and Signal Process. (ICASSP)"}
% @STRING{VTC            = "Proc. IEEE Vehic. Technol. Conf. (VTC)"}
% @STRING{ICC            = "Proc. IEEE Int. Conf. Commun. (ICC)"}
% @STRING{ISCAS          = "Proc. IEEE Int. Symp. on Circuits and Systems (ISCAS)"}
% @STRING{WCNC           = "Proc. IEEE Wireless Commun. and Netw. Conf. (WCNC)"}
% @STRING{ASILOMAR       = "Proc. Asilomar Conf. Signals, Systems and Computers (Asilomar)"}
% @STRING{PIMRC          = "Proc. IEEE Int. Symp. Personal Indoor and Mobile Radio Commun. (PIMRC)"}
% @string{GLOBECOM       = "Proc. IEEE Global Conmun. Conf. (GLOBECOM)"}
% @string{MILCOM         = "Proc. IEEE MILCOM"}
% @string{GlobalSIP      = "Proc. IEEE Global Conf. on Signal and Inform. Process. (GlobalSIP)"}
% @string{SPIE      = "Proc. SPIE"}

% IEEE Journals

% aerospace and military
% @STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
% @STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
% @STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
% @STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
% @STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
% @STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
% @STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
% @STRING{IEEE_J_IV         = "{IEEE} Trans. Intell. Veh."}
% @STRING{IEEE_J_TTE        = "{IEEE} Trans. Transport. Electrific."}
% @STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}
% @STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}



% circuits, signals, systems, audio and controls
% @STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
% @STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
% @STRING{IEEE_J_SYST       = "{IEEE} Syst. J."}
% @STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
% @STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
% @STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
% in 2014 ASL became ASLP
% @STRING{IEEE_J_ASLP       = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
% @STRING{IEEE_J_ASL        = "{IEEE} Audio, Speech, Language Process."}
% @STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
% @STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
% @STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
% @STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
% @STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
% @STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
% @STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
% @STRING{IEEE_J_ETCAS      = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
% @STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
% @STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
% @STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
% @STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
% @STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



% communications
% @STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
% @STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
% @STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
% @STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
% @STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}
% @STRING{IEEE_J_WCOML      = "{IEEE} Wireless Commun. Lett."}


% coding, data, information, knowledge
% @STRING{IEEE_J_BD         = "{IEEE} Trans. Big Data"}
% @STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
% @STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
% @STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}


% computers, computation, networking and software
% @STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
% @STRING{IEEE_J_ES         = "{IEEE} Embedded Syst. Lett."}
% @STRING{IEEE_J_IOT        = "{IEEE} Internet Things J."}
% @STRING{IEEE_J_XCDC       = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
% @STRING{IEEE_J_MMCT       = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
% @STRING{IEEE_J_SUSC       = "{IEEE} Sustain. Comput."}
% @STRING{IEEE_J_CC         = "{IEEE} Trans. on Cloud Comput."}
% @STRING{IEEE_J_CSS        = "{IEEE} Trans. Comput. Social Syst."}
% @STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
% @STRING{IEEE_J_CNS        = "{IEEE} Trans. Control Netw. Syst."}
% @STRING{IEEE_J_DSC        = "{IEEE} Trans. Depend. Sec. Comput."}
% @STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
% @STRING{IEEE_J_ETC        = "{IEEE} Trans. Emerg. Topics Comput."}
% @STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
% @STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% @STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
% @STRING{IEEE_J_MSCS       = "{IEEE} Trans. Multi-Scale Comput. Syst."}
% @STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
% @STRING{IEEE_J_NSE        = "{IEEE} Trans. Netw. Sci. Eng."}
% @STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
% @STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
% in 2012 NN became NNLS
% @STRING{IEEE_J_NNLS       = "{IEEE} Trans. Neural Netw. Learn. Syst."}
% @STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
% @STRING{IEEE_J_SC         = "{IEEE} Trans. Serv. Comput."}
% @STRING{IEEE_J_SIPN       = "{IEEE} Trans. Signal Inf. Process. Netw."}
% @STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}


% computer graphics, imaging, and multimedia
% @STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
% @STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
% @STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
% @STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}


% cybernetics, ergonomics, robots, man-machine, artificial intelligence and automation
% @STRING{IEEE_J_JAS        = "{IEEE/CAA} J. Autom. Sinica"}
% @STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
% @STRING{IEEE_J_AFFC       = "{IEEE} Trans. Affect. Comput."}
% @STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
% @STRING{IEEE_J_AMD        = "{IEEE} Trans. Auton. Mental Develop."}
% @STRING{IEEE_J_CCN        = "{IEEE} Trans. on Cogn. Commun. Netw."}
% in 2015 AMD became CDS
% @STRING{IEEE_J_CDS        = "{IEEE} Trans. Cogn. Develop. Syst."}
% @STRING{IEEE_J_CIAIG      = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
% in 2013 SMCB became CYB
% @STRING{IEEE_J_CYB        = "{IEEE} Trans. Cybern."}
% @STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
% @STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
% in 2013 SMCC became HMS
% @STRING{IEEE_J_HMS        = "{IEEE} Trans. Human-Mach. Syst."}
% @STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
% @STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
% in 1989 JRA became RA
% in August 2004, RA split into ASE and RO
% @STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
% @STRING{IEEE_J_RAL        = "{IEEE} Robot. Autom. Lett."}
% @STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
% @STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
% @STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
% @STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
% @STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
% in 2012 SMCA became SMCS
% @STRING{IEEE_J_SMCS       = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
% @STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}


% education, engineering, history, IEEE, professional
% @STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
% @STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
% @STRING{IEEE_J_RITA       = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
% @STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
% @STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
% @STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
% @STRING{IEEE_J_LT         = "{IEEE} Trans. Learn. Technol."}
% @STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}

% electromagnetics, antennas, EMI, magnetics and microwave
% @STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
% @STRING{IEEE_J_MAGL       = "{IEEE} Magn. Lett."}
% @STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
% @STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
% @STRING{IEEE_J_RFIC       = "{IEEE} {RFIC} J."}
% @STRING{IEEE_J_RFID       = "{IEEE} {RFID} J."}
% @STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
% @STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
% @STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
% @STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Techn."}
% @STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
% @STRING{IEEE_J_TTHZ       = "{IEEE} Trans. {THz} Sci. Technol."}
% @STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}


% industrial, commercial and consumer
% @STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}
% @STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
% @STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% @STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
% @STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
% @STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
% @STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
% @STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
% @STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
% @STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}

% instrumentation and measurement
% @STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}


% optics, lightwave and photonics
% @STRING{IEEE_J_JLT        = "J. Lightw. Technol."}
% @STRING{IEEE_J_OCN        = "{IEEE} J. Opt. Commun. Netw."}
% @STRING{IEEE_J_PJ         = "{IEEE} Photon. J."}
% @STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}


% sensors
% @STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}


% IEEE Magazines and Online Publications


% @STRING{IEEE_O_ACC        = "{IEEE} Access"}
% @STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
% @STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
% @STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
% @STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
% @STRING{IEEE_M_CHINAC     = "China Commun."}
% @STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
% @STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
% @STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
% @STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% @STRING{IEEE_O_CSTO       = "{IEEE} Commun. Surveys Tuts."}
% @STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
% CSEM changed to CSE in 1999
% @STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
% @STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
% @STRING{IEEE_M_C          = "Computer"}
% @STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
% @STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
% @STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
% @STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
% in 2012 DTC became DT
% @STRING{IEEE_M_DT         = "{IEEE} Des. Test"}
% @STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
% @STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
% @STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
% @STRING{IEEE_M_ETF        = "{IEEE} Electrific. Mag."}
% @STRING{IEEE_M_EMC        = "{IEEE} Electromagn. Compat."}
% @STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
% @STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
% @STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
% @STRING{IEEE_M_EXP        = "{IEEE} Expert"}
% @STRING{IEEE_M_GRS        = "{IEEE} Geosci. Remote Sens. Mag."}
% @STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
% @STRING{IEEE_M_IE         = "{IEEE} Ind. Electron. Mag."}
% @STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
% @STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
% @STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
% @STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
% @STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
% @STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
% @STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
% @STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
% @STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol. Mag."}
% @STRING{IEEE_M_NET        = "{IEEE} Netw."}
% IEEE's editorial manual lists "Pers. Commun.",
% but "Personal Commun. Mag." seems to be what is used in the journals
% @STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
% @STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
% @STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% @STRING{IEEE_M_PEL        = "{IEEE} Power Electron. Mag."}
% CAP and PER merged to form PE in 2003
% @STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
% @STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
% @STRING{IEEE_M_PULSE      = "{IEEE} Pulse"}
% @STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
% @STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
% @STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
% @STRING{IEEE_M_S          = "{IEEE} Softw."}
% @STRING{IEEE_M_SSC        = "{IEEE} Solid-State Circuits Mag."}
% @STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
% @STRING{IEEE_M_SMC        = "{IEEE} Syst., Man, Cybern. Mag."}
% @STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
% @STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
% @STRING{IEEE_M_WC         = "{IEEE} Wireless Commun."}


